SQUAD: Combining Sketching and Sampling Is Better than Either for Per-item Quantile Estimation

Stream monitoring is fundamental in many data stream applications, such as financial data trackers, security, anomaly detection, and load balancing. In that respect, quantiles are of particular interest, as they often capture the user's utility. For example, if a video connection has high tail latency, the perceived quality will suffer, even if the average and median latencies are low. In this work, we consider the problem of approximating the per-item quantiles. Elements in our stream are (ID, latency) tuples, and we wish to track the latency quantiles for each ID. Existing quantile sketches are designed for a single number stream (e.g., containing just the latency). While one could allocate a separate sketch instance for each ID, this may require an infeasible amount of memory. Instead, we consider tracking the quantiles for the heavy hitters (most frequent items), which are often considered particularly important, without knowing them beforehand. We first present a simple sampling algorithm that serves as a benchmark. Then, we design an algorithm that augments a quantile sketch within each entry of a heavy hitter algorithm, resulting in similar space complexity but with a deterministic error guarantee. Finally, we present SQUAD, a method that combines sampling and sketching while improving the asymptotic space complexity. Intuitively, SQUAD uses a background sampling process to capture the behaviour of the latencies of an item before it is allocated with a sketch, thereby allowing us to use fewer samples and sketches. Our solutions are rigorously analyzed, and we demonstrate the superiority of our approach using extensive simulations.

==> ACC_Psedocode.tex <==
%\newpage

\begin{comment}
\begin{algorithm}[t!]
	\caption{$ACC_k$}\label{alg:ACC}
	\scriptsize
	%\begin{multicols}{2}
	\begin{algorithmic}[1]
%		\ifdefined \NINEPAGES
		\Statex		Initialization: $%\BS \gets n^{1/k},
		 \OFFSET\gets 0, initialize\qquad \Tables, \incTables.$
		\Function {Add}{$x$}
			\For {$l \in 0,1,\ldots, k-1$}\Comment{Update all incomplete tables}
				\State $\incTables[l](x) += 1$
			\EndFor
		\EndFunction			
		\Function {EndBlock()}{}		
			\State $\OFFSET \gets (\OFFSET + 1) \mod n$
			\State $l \gets 0$
			\While {$((l\le k) \wedge (\OFFSET \mod n^{l/k} == 0))$} \Comment{End of a level $l$-segment}
				\If {$l \ne k$}
					\State $\Tables[l,\OFFSET] \gets \incTables[l]$
				\EndIf
				\If {$l \ge 1$}
					\State $empty \quad \incTables[l-1]$ \Comment{Delete all entries.}
				\EndIf
				\State $l \gets l + 1$
			\EndWhile
			\For {$l \in 1,2,\ldots, k-1$}
				\If {$\floor{n^{1/k}}^{l} \vert \OFFSET$}
				\State $\ghostTables[l] \gets \Tables[l,\OFFSET]$
				\EndIf
			\EndFor
		\EndFunction
		\Function {QueryTillSegment}{$x,\jmath$}
						\State $l_{min} \gets \max_{l} {{\floor{n^{1/k}}^{l} \vert \jmath}}$
						\State $l_{max} \gets {\floor{\log_{n^{1/k}} last}} - 1$
						\State $sum \gets 0$
						\If {$l_{min} = k$}
						\State $l_{max} \gets l_{min}$
						\EndIf
						\State $b \gets \jmath$
						\State $l \gets l_{min}$
						\While {$l \leq l_{max}$}
							\State $ sum += \Tables\brackets{l, b/ {\floor{n^{1/k}}}^{l}}(x) $
							\State $b \gets b -{\floor{n^{1/k}}}^{l}$
							\State $l \gets l + 1$
						\EndWhile
						\State \Return $sum$
		\EndFunction
		\Function {\SIQ}{$x,\ell,\jmath$}		
			\State $last = (\OFFSET - \jmath) \mod n$ \Comment{The index of the most recent block}
			\State $first = (\OFFSET - \ell) \mod n$ \Comment{The index of the oldest queried block}		
			\State $sum \gets 0$
			\If {$last \ge first$}
				\State \Return $\mbox{\Call {QueryTillSegment} {x, last}} - 	\mbox{\Call {QueryTillSegment} {x, first}}$
			\EndIf
			\State $sum \gets \mbox{\Call {QueryTillSegment} {x, last}} + \mbox{\Call {QueryTillSegment} {x, n}}$
			\State $location \gets first - 1$
			\State $tmp \gets 0$
			\State $l \gets \max_{l} {{\floor{n^{1/k}}^{l} \vert location}}$
			\While {$l \leq k - 1$}
				\While {$location \ge \offset + 1$}
					\State $tmp +=  \Tables\brackets{l, location/ {\floor{n^{1/k}}}^{l}}(x)$
					\State $l \gets l + 1$
					\State $location \gets {\floor{n^{1/k}}}^{l} * \floor{location/ {\floor{n^{1/k}}}^{l}}$
				\EndWhile
				\State $tmp += \ghostTables[l]$
				\State $l \gets l + 1$
			\EndWhile
			\State \Return $sum - tmp$
		\EndFunction		
	\end{algorithmic}
	%\end{multicols}
	\normalsize
\end{algorithm}
\end{comment}
\ifdefined\NINEPAGES
\vspace*{-5mm}
%\setlength{\textfloatsep}{0pt}
%\setlength{\intextsep}{0pt}
%\setlength{\dbltextfloatsep}{0pt}
%\setlength{\abovedisplayskip}{0pt}
%\setlength{\belowdisplayskip}{0pt}
\fi
\begin{algorithm}[t]
	\caption{$ACC_k$}\label{alg:ACC}
	\ifdefined\VLDB
	\scriptsize
	\fi
%\small
	%\begin{multicols}{2}
	\begin{algorithmic}[1]
		%		\ifdefined \NINEPAGES
		\Statex		Init: $%\BS \gets n^{1/k},
		\OFFSET\gets 1,
		\tableDis\triangleq {n^{1/k}},$\\
%		\tableDis\triangleq \floor{n^{1/k}},		
		\qquad{} $initialize\qquad \Tables, \incTables, \ghostTables$
		\Function {Add}{$x$}
		\For {$\ell \in 0,1,\ldots, k-1$}\Comment{Update all incomplete tables}
		\State $\incTables[\ell](x) += 1$
		\EndFor
		\EndFunction			
		\Function {EndBlock()}{}		
		\State $\ell \gets 0$
		\While {$((\ell < k - 1) \wedge \OFFSET \mod \tableDis^{\ell+1} = 0)$}
		\Statex\Comment{A Level-$\ell$ block has ended}
			\State $empty \ \incTables[\ell], \ghostTables[\ell]$ \Comment{Delete all entries}
			\State $\ell \gets \ell + 1$
%		\While {$((\ell\le k) \wedge (\OFFSET \mod n^{\ell/k} == 0))$} \Comment{End of a level $l$-segment}		
		\EndWhile
%		\If {$\OFFSET \mod \tableDis = 0$}
%			\State $\ell \gets 0$
%		\EndIf
		\State $\ghostTables[\ell] \gets \Tables[\ell,\OFFSET]$ \label{line:ghost_table}	
		\State $\Tables[\ell,\OFFSET] \gets \incTables[\ell]$\Comment{Copy Table}
		\If {$\OFFSET = n$} \Comment{New frame}
			\State $empty \ \incTables[k-1], \ghostTables[k-1]$
%			 \Comment{Reset all~entries}			
		\EndIf
		\State $\OFFSET \gets 1 + (\OFFSET \mod n)$		
		\EndFunction
		\Function {\windowQuery{}}{}\Comment{Frequency in the last $w$ blocks}\label{func:winQuery}
			\State \resizebox{7.45cm}{!}{{\scriptsize $\curFrameFreq\gets incTables[0](x) + \sum_{\ell=1}^{\log_{\tableDis}\OFFSET} \Tables\brackets{\ell, \tableDis^{\ell}\floor{\frac{\OFFSET}{\tableDis^{\ell}}}}(x)$}\small \label{line:sum_tables}}
			\If {$w\le \OFFSET + 1$}
				\State\Return \resizebox{6.1cm}{!}{{\scriptsize $\curFrameFreq - \sum_{\ell=0}^{\log_{\tableDis}\OFFSET+1-w} \Tables\brackets{\ell, \tableDis^{\ell}\floor{\frac{\OFFSET+1-w}{\tableDis^{\ell}}}}(x)$}} \label{line:fixed_result}
			\EndIf
			\State $B \gets n+\OFFSET+1-w$ \label{line:case2_begin}
			\State $L \gets \max\set{\ell\mid \tableDis^{\ell}\floor{\frac{B}{\tableDis^{\ell}}}\ge \OFFSET+1}$
			%\State {\tiny$preW \gets \sum_{\ell=0}^{L} \Tables\brackets{\ell, \tableDis^{\ell}\floor{\frac{B}{\tableDis^{\ell}}}}(x) + \sum_{\ell=L+1}^{k-1} \ghostTables[\ell](x)$}
			\State {\tiny$preW \gets \sum_{\ell=0}^{L} \Tables\brackets{\ell, \tableDis^{\ell}\floor{\frac{B}{\tableDis^{\ell}}}}(x) + \sum_{\ell=L+1}^{k-1} \ghostTables[\ell](x)$}
			\small
			\State\Return $\curFrameFreq+\Tables[k-1,n](x) - preW$ \label{line:case2_end}
%			-sum_{\ell=0}^{\log_{\tableDis}\OFFSET-w} \Tables\brackets{\ell, \tableDis^{\ell}\floor{\frac{\OFFSET-w}{\tableDis^{\ell}}}}(x) - sum_{\ell=L+1}^{k} \ghostTables[\ell](x)$
		\EndFunction
		\Function {\SIQ}{$x,i,j$}		
		\If {$i = 0$} \label{line:case1}
			\State \Return \windowQueryText{}$(x,j)$
		\EndIf
		\State \Return \windowQueryText{}$(x,j)$ - \windowQueryText{}$(x,i)$
%		\State $last = 1 + ((\OFFSET - \jmath) \mod n)$ \Comment{The index of the most recent block}
%		\State $first = 1 + ((\OFFSET - \ell) \mod n)$ \Comment{The oldest queried block}		
%%		\State $sum \gets 0$
%		\If {$last \ge first$} \Comment{if contained in the current frame}
%		\State \Return
%%$\mbox{\Call {TillBlock} {x, last}} - 	\mbox{\Call {TillBlock} {x, first}}$
%%		$$\sum_{\ell=0}^{\log_{\tableDis}first} \Tables\brackets{\ell, n^{\ell/k}\floor{\frac{first}{n^{\ell/k}}}}(x) - \sum_{\ell=0}^{\log_{\tableDis}last} \Tables\brackets{\ell, n^{\ell/k}\floor{\frac{last}{n^{\ell/k}}}}(x) $$
%		$$\sum_{\ell=0}^{\log_{\tableDis}first} \Tables\brackets{\ell, \tableDis^{\ell}\floor{\frac{first}{\tableDis^{\ell}}}}(x) - \sum_{\ell=0}^{\log_{\tableDis}last} \Tables\brackets{\ell, \tableDis^{\ell}\floor{\frac{last}{\tableDis^{\ell}}}}(x) $$
%		\EndIf
%		\State $maxL = \max\set{\ell\mid (first-1)/\tableDis^{\ell}\ge \OFFSET+1}$
%		\State $tillFirst\gets \sum_{\ell=0}^{\log_{\tableDis} first-1} \Tables\brackets{\ell, \tableDis^{\ell}\floor{\frac{last}{\tableDis^{\ell}}}}(x)$
%		\State $sum \gets \mbox{\Call {TillBlock} {x, last}} + \mbox{\Call {TillBlock} {x, n}}$
%		\State $location \gets first - 1$
%		\State $tmp \gets 0$
%		\State $l \gets \max_{l} {{\tableDis^{l} \vert location}}$
%		\While {$l \leq k - 1$}
%		\While {$location \ge \\OFFSET + 1$}
%		\State $tmp +=  \Tables\brackets{l, location/ {\tableDis}^{l}}(x)$
%		\State $l \gets l + 1$
%		\State $location \gets {\tableDis}^{l} * \floor{location/ {\tableDis}^{l}}$
%		\EndWhile
%		\State $tmp += \ghostTables[l]$
%		\State $l \gets l + 1$
%		\EndWhile
%		\State \Return $sum - tmp$
		\EndFunction		
{}	\end{algorithmic}
	%\end{multicols}
	\normalsize
\end{algorithm}
\ifdefined\NINEPAGES
\setlength{\textfloatsep}{14pt}
\setlength{\intextsep}{16pt}
\setlength{\dbltextfloatsep}{12pt}
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
\fi

==> background.tex <==
%\subsection{Background}

High-performance stream processing is essential for many applications such as financial data trackers, intrusion-detection systems, network monitoring, and sensor networks.
Such applications require algorithms that are both time and space efficient to cope with high-speed data streams.
Space efficiency is needed, due to the memory hierarchy structure, to enable cache residency and to avoid page swapping. This residency is vital for obtaining good performance, even when the theoretical computational cost is small (e.g., constant time algorithms may be inefficient if they access the DRAM for each element).
To that end, stream processing algorithms often build compact approximate \emph{sketches} (synopses) of the input streams.
%As a trade-off, these sketches answers approximate query with guarantees on specific error.

Recent items are often more relevant than old ones, which requires an aging mechanism for the sketches.
Many applications realize this by tracking the stream's items over a \emph{sliding window}.
That is, the sliding window model~\cite{DatarGIM02} considers only a window of the most recent items in the stream,  while older ones do not affect the quantity we wish to estimate.
Indeed, the problem of maintaining different types of sliding window statistics \mbox{was extensively studied~\cite{ArasuM04,WCSS,DatarGIM02,papapetrou2015sketching,LeeT06}.}

Yet, sometimes the window of interest may not be known a priori \changed{or they may be multiple interesting windows~\cite{dallachiesa2013identifying}}.
Further, the ability to perform drill-down queries, in which we examine the behavior of the system in finer and finer granularity may also be beneficial, especially for security applications.
For example, this enables detecting when precisely a particular anomaly has started and who was involved in it~\changed{\cite{Estan2002}}.
Additional applications for this capability include identifying the sources of flash crowd effects and pinpointing the cause-effect relation surrounding a surge in demand on an e-commerce website~\changed{\cite{ecommerce}}.

In this work, we study a model that allows the user to specify an interval of interest at query time.
This extends traditional sliding windows that only consider fixed sized windows.
%where the measurement is done with regards to a fixed sized window.
As depicted in Figure~\ref{fig:overview}, a sub-interval of a maximal window is passed as a parameter for each query, and the goal of the algorithm is to reply correspondingly.
Naturally, one could maintain an instance of a sliding window algorithm for each possible interval within the maximal sliding window.
Alas, this is both computationally and space inefficient.
\mbox{Hence, the challenge is to devise efficient solutions.}

This same model was previously explored in~\cite{papapetrou2015sketching}, which based their solution on \emph{exponential histograms}~\cite{DatarGIM02}.
However, as we elaborate below, their solution is both memory wasteful and computationally inefficient.
Further, they only provide probabilistic guarantees.


%\emph{Heavy hitters} are network flows that consume a significant percentage of the total network bandwidth.
%Identifying such flows is essential for many applications.
%For example, a load balancer could use a sophisticated scheduling algorithm for the heavy hitters, while resorting to a random allocation for all other flows.
%Since by definition the number of heavy hitters is small, such a balancing scheme is much more computationally efficient than trying to optimize the allocation of all flows.
%Similarly, bandwidth enforcement is only important for the heavy hitters, a large number of network security attacks are associated with heavy hitters, etc.
%
%
%
%Further, since the recent characteristics of the various flows are typically more relevant than old historical behavior, it is important to track the heavy hitters over a \emph{sliding window}.
%
%Indeed, the problem of finding heavy hitters over sliding windows was extensively studied~\cite{HungLT10,WCSS,ArasuM04,LeeT06}.
%Yet, sometimes the window of interest is not known apriori.
%
%
%Further, the ability to perform drill-down queries, in which the behavior of the network can be examined in finer and finer granularities may also be beneficial, especially for network security applications.
%For example, this enables detecting when precisely a particular anomaly has started and who was involved in it.
%
%In this work, we study a model that allows the user to specify an interval of interest in query time.  This extends traditional sliding windows where the measurement is done with regards to a fixed sized window.
%
%As depicted in Figure~\ref{fig:overview}, a sub-interval of a maximal window is passed as a parameter for each query and the goal
%%of the algorithm
%is to reply in a corresponding manner.
%
%
%Naturally, one could maintain an instance of a sliding window algorithm for each possible interval within the maximal sliding window.
%However, is both computationally and space inefficient.
%Hence, the challenge is to come up with efficient solutions.
%
%This model was previously explored in~\cite{papapetrou2015sketching}, which based their solution on \emph{exponential histograms}~\cite{DatarGIM02}.
%However, their solution is both memory wasteful and computationally inefficient.
%Further, they only provide probabilistic guarantees.


==> contributions.tex <==
\subsection*{Contributions}

\begin{table*}[t]
	\scriptsize
	\addtolength{\tabcolsep}{-0pt} \addtolength{\parskip}{-0.1mm} 
	\centering{
	%\resizebox{\textwidth}{!}{
		\begin{tabular}{|@{}c@{}|c|c|c|c|>{\tiny}c|}
			\hline
			Algorithm & Space &  Update Time & Query Time & Comments\tabularnewline
			\hline
			\hline
			WCSS ~\cite{WCSS}& $O(\eps^{-1}\log (W|\mathcal U|))$ & $O(1)$ & $O(1)$ & Only supports fixed-size window queries.
			\tabularnewline
			\hline
			ECM ~\cite{papapetrou2015sketching}& $O(\eps^{-2}\log W\log\delta^{-1})$ & $O(\log\delta^{-1})$ & $O(\eps^{-1}\log W\log\delta^{-1})$ & Only provides probabilistic guarantees.\tabularnewline
			\hline
			RAW & $O(\eps^{-2}\log (W|\mathcal U|))$ & $O(\oneOverE)$ & $O(1)$ & Uses prior art (WCSS) as a black box.\tabularnewline
			\hline
			\multirow{3}{*}{ACC$_k$} & \multirow{1}{*}{\hspace{-15mm}$O\Big(\oneOverE\log (W|\mathcal U|)$} & \multirow{3}{*}{$O(k+\eps^{-2}/W)$} & \multirow{3}{*}{$O(k)$} & Constant time operations for \tabularnewline
            & $+k\eps^{-(1+1/k)} \log\oneOverE\Big)$& & & $k=O(1)\wedge \eps=\Omega(W^{-1/2})$.\tabularnewline
			\hline
%\ifdefined\EXTENDED		
%			HIT & $O(\oneOverE(\log W + \log|\mathcal U|))$ & $O(1 + \log \oneOverE\cdot \oneOverE/W)$ & $O(\log \oneOverE)$ & A logarithmic factor from optimal space.\tabularnewline & & & & $O(1)$ time updates when $\eps=\Omega\parentheses{\frac{\logw}{W}}$.
%\fi
%\ifdefined\NINEPAGES
			\multirow{3}{*}{HIT} & \multirow{3}{*}{$O(\eps^{-1}(\log (W|\mathcal U|) + \log^2\oneOverE))$} & \multirow{3}{*}{\changed{$O(1 + \parentheses{\oneOverE\cdot\log{ \oneOverE} }/W)$}} & \multirow{3}{*}{$O(\log \oneOverE)$} & Optimal space when $\log^2\oneOverE=O(\log (W|\mathcal U|))$,
			\tabularnewline & & & &
			 $O(1)$ time updates when $\eps=\Omega\parentheses{\frac{\logw}{W}}$.
%\fi	
			\tabularnewline
			\hline
		\end{tabular}
		\normalsize	
		{{\caption{Comparison of the algorithms proposed in the paper with ECM and WCSS (that solves the simpler problem of fixed-size windows). ACC$_k$ can be instantiated for any $k\in\mathbb N$.
\ifdefined\NINEPAGES
\vspace*{-0.2cm}
\fi				
						}
				\label{tbl:comparison}
	}}}
\end{table*}
%\section{Contributions}

\begin{figure}[t]
	%\medskip
	\centering
	%\frame{
	\includegraphics[width=\linewidth]{overview.png}
	%}
	\vspace{-8mm}	\caption{\small{
    We process items and support frequency queries within an interval specified at query time.
    While the traditional sliding window model can answer queries for a \emph{fixed window}, our approach allows us to consider \emph{any} interval that is contained within the last $W$ items.
    In this example, we ask about the frequency of the item $a$ within the interval $[8,18]$. If we allow an additive error of $2$, the answer to this query should be in the range $[4, 6]$.}
	}
	%\caption{\small{We process items and support frequency queries within an interval specified at query time.
%	While previous work can answer queries for a \emph{fixed window}, our approach allows \emph{any} interval that is contained in the last $W$ packets to be queried.
	%While the traditional sliding window model can answer queries for a \emph{fixed window}, our approach allows us to consider \emph{any} interval that is contained within the last $W$ items.
	%In this example, assuming that we allow an additive error of $1$, we ask about the frequency of item $a$ within the interval $[8,18]$. The answer to this query should be in the range $[4, 5]$.}
	%}
	\label{fig:overview}
	\vspace{-3mm}
\end{figure}
\normalsize

Our work focuses on the problem of estimating frequencies over an ad-hoc interval given at query time. 
We start by introducing a formal definition of this generalized estimation problem nicknamed \IFProblem{}.
%and \IHHProblem.

To systematically explore the problem, we first present a na\"{\i}ve strawman algorithm (RAW), which uses multiple instances of a state-of-the-art fixed window algorithm.
%\ifdefined\EXTENDED
In such an approach, an interval query is satisfied by querying the instances that are closest to the beginning and end of the interval and then subtracting their results.
This algorithm is memory wasteful and its update time is slow, but it serves as a baseline for comparing our more sophisticated solutions.
%\fi
%\ifdefined\NINEPAGES
%It serves as a baseline for comparing our more sophisticated solutions.
%\fi
Interestingly, RAW achieves constant query time while the previously published ECM algorithm~\cite{papapetrou2015sketching} answers queries in $O(\eps^{-1}\log W\log\delta^{-1})$, where $W$ is the maximal window size and $\delta$ is the probability of failure. Additionally, it requires about the same amount of memory and is \mbox{deterministic while ECM has an error probability.}
%Moreover, RAW performs updates in $O(\oneOverE)$ and ECM in $O(\log\delta^{-1})$.

While developing our advanced algorithms, we discovered that both intrinsically solve a common problem that we nickname \SIProblem.
Hence, our next contribution is in identifying and formally defining the \SIProblem{} problem and showing a reduction from \SIProblem{} to the \IFProblem{} problem.
This makes our algorithms shorter, simpler, and easier to prove, \mbox{analyze and implement.}

Our algorithms, nicknamed \emph{HIT} and $ACC_k$ (to be precise, $\set{ACC_k}_{k\ge 1}$ is a family of algorithms), process items in constant time (under reasonable assumptions on the error target) -- asymptotically faster than RAW.
HIT is asymptotically memory optimal while serving queries in logarithmic time.
Conversely, $ACC_k$ answers queries in constant time and incurs a sub-quadratic space overhead.
%We formally prove the correctness and space analysis of our


We present formal correctness proofs as well as space and runtime analysis.
We summarize our solutions' asymptotic performance in Table~\ref{tbl:comparison}.


Our next contribution is a performance evaluation study of our various algorithms along with ($i$) ECM-Sketch ~\cite{papapetrou2015sketching}, the previously suggested solution for interval queries and ($ii$) the state-of-the-art \emph{fixed window} algorithm (WCSS)~\cite{WCSS}, which serves as a best case reference point since it solves a more straightforward problem.
We use on real-world packet traces from Internet backbone routers, from a university datacenter, and from a university's border router.
Overall, our methods (HIT and ACC$_k$) process items $75$--$2000$ times faster and consume at least $20$ times less space than the naive approach (RAW) while requiring a similar amount of memory as the state-of-the-art \emph{fixed size window} algorithm (WCSS).
Compared to the previously known solution to this problem (ECM-Sketch~\cite{papapetrou2015sketching}), all our advanced algorithms are both faster and more space efficient.
In particular, our fastest algorithm, ACC$_1$, processes items $90$--$250$ times faster than ECM-Sketch, serves queries at least $730$ times quicker and consumes at least $40\%$ less~space.

Last, we extend our results to time-based intervals, heavy hitters~\cite{MG,berinde2010space}, hierarchical heavy hitters~\cite{CormodeHHH,Hershberger2005}, and for detecting traffic volume heavy-hitters~\cite{DIM-SUM}, i.e., when counting each flow's total traffic rather than item count.
We also discuss applying our algorithms in a distributed settings, in which measurements are recorded independently by multiple sites (e.g., multiple routers), and the goal is to obtain a global network analysis.


==> datasetTable.tex <==
\ifdefined \NINEPAGES

\fi
% \begin{table*}[t]
% 	\addtolength{\tabcolsep}{-0pt} \addtolength{\parskip}{-0.1mm} \center{
% 		\begin{tabular}{|c|c|c|c|c|c|c|c|}
% 			\hline
% 			Trace &Date(Y/M/D) &  \#Packets & Total volume & Mean size & Max size & \% large packets  & \% large packet traffic\tabularnewline
% 			\hline
% 			\hline
% 			Chicago16 & 2016/02/18 & 97 M & 94 GB & 1046 & 49458 & 0.34\% & 0.5\%\tabularnewline
% 			\hline
% 			Chicago15 & 2015/12/17 & 85 M & 80 GB & 1013 & 64134 & 0.22\%  & 0.34\%\tabularnewline
% 			\hline
% 			SanJose14 & 2014/06/19 & 112 M & 149 GB & 1424 & 65535 & 0.78\% & 25.02\%\tabularnewline
% 			\hline
% 			SanJose13 & 2013/12/19 & 97 M & 110 GB & 1225 & 65528 & 0.49\% & 18.81\% \tabularnewline
% 			\hline
% 		\end{tabular}
% 		
% 		{{\caption{A summary of key characteristics of the real Internet traces used in this work. }
% 				\label{tbl:traces}
% 			}}}
% 		\end{table*}
\normalsize 

==> intro.tex <==
\section{Introduction}
\label{sec:intro}

\input{background}
\input{contributions}

\paragraph*{Paper roadmap}
We briefly survey related work in Section~\ref{sec:related}.
We state the formal model and problem statement in Section~\ref{sec:prelim}.
Our first algorithm RAW is described in Section~\ref{windows-sizes}.
We present the auxiliary \SIProblem{} problem, which both our advanced algorithms solve and has a simple reduction to the \IFProblem{} problem, in Section~\ref{sec:block-interval}.
The improved algorithms, \emph{HIT} and $ACC_k$, are then described in Section~\ref{sec:improved_algos}.
The performance evaluation of our algorithms and their comparison to ECM-Sketch and WCSS is detailed in Section~\ref{sec:eval}.
Section~\ref{sec:extensions} discusses extensions of our work.
%We present the extensions of our work in Section~\ref{sec:extensions}.
Finally, we conclude with a discussion in Section~\ref{sec:discussion}.

\input{related-work}


